Limiting aspects of non-convex ${TV}^\phi$ models

Recently, non-convex regularisation models have been introduced in order to provide a better prior for gradient distributions in real images. They are based on using concave energies $\phi$ in the total variation type functional ${TV}^\phi(u) := \int \phi(|\nabla u(x)|) d x$. In this paper, it is demonstrated that for typical choices of $\phi$, functionals of this type pose several difficulties when extended to the entire space of functions of bounded variation, ${BV}(\Omega)$. In particular, if $\phi(t)=t^q$ for $q \in (0, 1)$ and ${TV}^\phi$ is defined directly for piecewise constant functions and extended via weak* lower semicontinuous envelopes to ${BV}(\Omega)$, then still ${TV}^\phi(u)=\infty$ for $u$ not piecewise constant. If, on the other hand, ${TV}^\phi$ is defined analogously via continuously differentiable functions, then ${TV}^\phi \equiv 0$, (!). We study a way to remedy the models through additional multiscale regularisation and area strict convergence, provided that the energy $\phi(t)=t^q$ is linearised for high values. The fact, that this kind of energies actually better matches reality and improves reconstructions, is demonstrated by statistics and numerical experiments.

==> highlightname.tex <==
%\addbibresource{\jobname.bib}
\newcommand*{\mknamesignature}[5]{\def#1{#2|#3|#4|#5}}
\mknamesignature{\highlightname}{Valkonen}{Tuomo}{}{}
% mbox needed to not make next character automatically  upper case
\def\shortform{\mbox{\textsl{T.V.}}}
\makeatletter

\DeclareNameFormat{labelname}{%
  \begingroup
  \mknamesignature{\currentsignature}{#1}{#3}{#5}{#7}%
  \ifdefequal{\highlightname}{\currentsignature}%
    {\let\mkbibnamefirst=\@gobble%
     \def\mkbibnamelast{\shortform\@gobble}%
     \let\mkbibnameprefix=\@gobble%
     \let\mkbibnameaffix=\@gobble}%
    {\let\mkbibnamefirst=\@gobble}%
  \ifcase\value{uniquename}%
    \usebibmacro{name:last}{#1}{#3}{#5}{#7}%
  \or
    \ifuseprefix
      {\usebibmacro{name:first-last}{#1}{#4}{#5}{#8}}
      {\usebibmacro{name:first-last}{#1}{#4}{#6}{#8}}%
  \or
    \usebibmacro{name:first-last}{#1}{#3}{#5}{#7}%
  \fi
  \endgroup
  \usebibmacro{name:andothers}%
}

\makeatother


==> removed.tex <==
    Let us then consider the Cantor part in \eqref{eq:grad-u-epsilon-split}.
    We observe that $\int_{\R^m} \rho_\epsilon(x-y) \d \abs{D^c u_0(y)}=0$,
    for $x \in \R^m \setminus K$. Moreover $\abs{D^c u_0}(\BD \Omega)=0$
    because $\BD \Omega$ is Lipshitz and hence $\sigma$-additive with respect
    to $\H^{m-1}$. Thus we get for $\epsilon \in (0, 1)$ the estimate
    \TODO{Covering theorems help to get rid of $K$ dep.?}
    \TODO{full bs:}
    \begin{equation}
        \label{eq:tvqc-cantor-estim}
        \int_{\R^m} \phi\left(\int_{\R^m} \rho_\epsilon(x-y) \d \abs{D^c u_0}(y)\right) \d x
        \le
        \int_{K} \phi\left(\abs{D^c u_0}(K)\right) \d x
        =
        \L^m(K) \phi\left(\abs{D^c u}(\Omega)\right) \d x.
    \end{equation}

    The procedure for the jump part in \eqref{eq:grad-u-epsilon-split} is similar
    to the Cantor part, but slightly more refined. By the countable $\H^{m-1}$-rectifiability 
    of the jump set $J_{u_0}$, we may find Lipschitz $\{\gamma_k: \R^{m-1} \to \R^m\}_{k=1}^\infty$
    such that $\H^{m-1}(J_{u_0} \setminus \Union_{k=1}^\infty \Gamma_k)=0$ 
    with $\Gamma_k \defeq \gamma_k(\R^{m-1})$.
    %We may further assume that $\H^{m-1}(\Gamma_k) \le 1$ by breaking the graphs $\Gamma_k$
    %into smaller parts if necessary. 
    Given $\delta > 0$, we may find an index $N$ such that
    \[
        \abs{D^j u_0}\left(J_{u_0} \setminus \Union_{k=1}^N \Gamma_k\right) \le \delta/2.
    \]
    Moreover, since $\theta_{u_0} \in L^1(J_u)$, where $\abs{D^j u_0} = \theta_{u_0} \H^{m-1} \restrict J_u$,
    we find a Borel set $U \subset J_u$ and $M >0$ such that
    \begin{equation}
        \label{eq:u-set-def}
        \sup_{x \in U} \theta_{u_0}(x) < M
        \quad
        \text{and}
        \quad
        \abs{D^j u_0}\left(J_u \isect \Union_{k=1}^N (\Gamma_k \setminus U)\right) \le \delta/2.
    \end{equation}
    Setting $J^\delta \defeq J_{u_0} \setminus \Union_{k=1}^N (\Gamma_k \isect U)$,
    we then have $\abs{D^j u_0}(J^\delta) \le \delta$, and for $\epsilon \in (0, 1)$ we get as
    for the Cantor part that
    \TODO{full bs:}
    \[
        \int_{\R^m} \phi\left(\int_{\R^m} \rho_\epsilon(x-y) \d \abs{D^j u_0 \restrict J^\delta}(y)\right)
        \le
        \int_{K} \phi\left(\abs{D^j u_0 \restrict J^\delta}(K)\right) \d x
        \le
        \L^m(K) \phi(\delta).
    \]
    With respect to $\Gamma_k \isect U$ we set
    \[
        V_{k,\epsilon} \defeq K \isect \bigl(\Gamma_k +\B(0, \epsilon)\bigr),
    \]
    and observe that
    \[
        \H^{m-1}(\Gamma_k \isect \B(x, \epsilon))
        \le \chi_{V_{k,\epsilon}}(x) \epsilon^{m-1} c_k.
    \]
    Therefore
    \[
        \begin{aligned}
        \int_{\R^m} \rho_\epsilon(x-y) \d \abs{D^j u_0 \restrict (\Gamma_k \isect U)}(y)
        &
        \le
        \epsilon^{-m} \abs{D^j u_0}(\Gamma_k \isect U \isect \B(x, \epsilon))
        \\
        &
        \le
        \epsilon^{-m} M \H^{m-1}(\Gamma_k \isect \B(x, \epsilon))
        &
        &
        \text{(by \eqref{eq:u-set-def})}
        \\
        &
        \le
        \chi_{V_{k,\epsilon}}(x)
        M c_k \epsilon^{-1}.
        \end{aligned}
    \]
    An application of the coarea formula shows that 
    \[
        \L^m(V_{k,\epsilon}) \le C_k \epsilon
    \]
    where $C_k$ again dependent on the Lipschitz factor of $\gamma_k$ and on the diameter of $K$.
    Thus
    \[
        \int_{\R^m} \phi\left(\int_{\R^m} \rho_\epsilon(x-y) \d \abs{D^j u_0 \restrict (\Gamma_k \isect U)}(y)\right) \d x
        \le
        \int \chi_{V_{k,\epsilon}} \phi(M c_k \epsilon^{-1}) \d x
        \le
        C_k \epsilon \phi(M c_k \epsilon^{-1}).
    \]
    But, using the fact that $\phi(t)/t \to 0$ as $t \to \infty$, we obtain
    \[
        %\lim_{\epsilon \downto 0} \int_{\R^m} \phi\left(\int_{\R^m} \rho_\epsilon(x-y) \d \abs{D^j u_0 \restrict \Gamma_k}(y)\right) \d x = 0.
        \lim_{\epsilon \downto 0} C_k \epsilon \phi(M c_k \epsilon^{-1}) = 0.
    \]
    Thus, approximating $\abs{D^j u_0} \le \sum_{k=1}^N \abs{D_j u_0 \restrict (\Gamma_k \isect U)} + \abs{D_j u_0 \restrict J^\delta}$,
    we obtain
    \[
        \begin{split}
        \liminf_{\epsilon \downto 0}
        \int_{\R^m} \phi\left(\int_{\R^m} \rho_\epsilon(x-y) \d \abs{D^j u_0}(y)\right) \d x
        &
        \le
        \liminf_{\epsilon \downto 0}
        C_k \epsilon \phi(M c_k \epsilon^{-1})
        +
        \L^m(K) \phi(\delta)
        \\
        &
        =
        \L^m(K) \phi(\delta).
        \end{split}
    \]
    As $\delta > 0$ was arbitrary and $\phi(\delta) \to$ as $\delta \downto 0$, we conclude that
    \begin{equation}
        \label{eq:tvqc-jump-estim}
        \lim_{\epsilon \downto 0}
        \int_{\R^m} \phi\left(\int_{\R^m} \rho_\epsilon(x-y) \d \abs{D^j u_0}(y)\right) \d x = 0.
    \end{equation}


==> symbols-ip.tex <==

\usepackage{undertilde}

\newcommand{\jprod}{\circ}
\newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\iK}{\interior \K}
\newcommand{\E}{\mathcal{E}}
\newcommand{\Neigh}{\mathcal{C}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\nullspace}[1]{\mathcal{N}(#1)}
\newcommand{\iprod}[2]{\langle #1,#2\rangle}
\newcommand{\Pep}{P_e^\perp}
\newcommand{\DC}{\mathrm{DC}}
\newcommand{\extsubdiff}{\widehat \subdiff}
\newcommand{\subdiffDC}{\subdiff^\DC}
\newcommand{\extsubdiffDC}{\extsubdiff^\DC}
\newcommand{\polar}[1]{{#1}^\circ}
\newcommand{\bipolar}[1]{{#1}^{\circ\circ}}
\newcommand{\regnormal}{\widehat N}
\newcommand{\regtangent}{\widehat T}
\newcommand{\HG}{{\widehat G}}
\newcommand{\HU}{{\widehat U}}
\newcommand{\IG}{\inv G}
\newcommand{\IHG}{\inv \HG}
\newcommand{\varsym}{\bullet}
\newcommand{\wtilde}{\widetilde}
\newcommand{\setto}{\rightrightarrows}

\renewcommand{\norm}[1]{\|#1\|}
\newcommand{\adjnorm}[1]{\left\|#1\right\|}

\newcommand{\eigval}{\zeta}
\newcommand{\eigvaltwo}{\sigma}

\newcommand{\Arw}{\mathrm{Arw}}


==> symbols-mna.tex <==

\newcommand{\mna}{\phi}
\newcommand{\plusmna}{\oplus}
\newcommand{\minusmna}{\ominus}
\newcommand{\iprodmna}{\odot}
%\DeclareMathOperator{\plusmna}{\hat +}
%\DeclareMathOperator{\minusmna}{\hat{--}}
%\DeclareMathOperator{\iprodmna}{\hat \times}
\newcommand{\Rmna}{\R_\mna}
\newcommand{\maybeeq}{\stackrel{?}{=}}
\newcommand\rhodom\sqsubset
\newcommand\rhodominv\sqsupset
\newcommand\rhodomneq{\sqsubset_{!}}
\newcommand\rholub\sqcup
\newcommand\rhoglb\sqcap
\newcommand{\sumop}{\biguplus}
\newcommand{\sumz}{\biguplus}
\newcommand{\plusz}{\uplus}
\newcommand{\minusz}{\uminus}
\newcommand{\pz}{\zeta}

